Structure-Preserving Instance Segmentation via Skeleton-Aware Distance Transform

Objects with complex structures pose significant challenges to existing instance segmentation methods that rely on boundary or affinity maps, which are vulnerable to small errors around contacting pixels that cause noticeable connectivity change. While the distance transform (DT) makes instance interiors and boundaries more distinguishable, it tends to overlook the intra-object connectivity for instances with varying width and result in over-segmentation. To address these challenges, we propose a skeleton-aware distance transform (SDT) that combines the merits of object skeleton in preserving connectivity and DT in modeling geometric arrangement to represent instances with arbitrary structures. Comprehensive experiments on histopathology image segmentation demonstrate that SDT achieves state-of-the-art performance.

==> tex-fig/fig_qual.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{fig/supp_qual.png}
    \caption{Qualitative comparison on the gland segmentation dataset. From left to right, we show ({\bf a}) histopathology image, ({\bf b}) groundtruth segmentation masks, ({\bf c}) prediction of distance transform (DT) trained with cross-entropy (CE) loss, ({\bf d}) prediction of \sdt trained with L1 regression loss, and ({\bf e}) prediction of \sdt trained with CE loss. For non-convex objects with thin connections (first 3 rows), our \sdt w/ CE loss can better preserve connectivity in comparison with DT, and produce sharper energy landscape than \sdt w/ L1 loss. DT and \sdt perform equally well on convex objects (the last row). 
    }\label{fig:supp_qual}
\end{figure*}

==> tex-tab/tab_gland.tex <==
\begin{table}[t]
    \begin{center}
    \resizebox{0.5\columnwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{Method} &  \multicolumn{2}{c}{F1 Score $\uparrow$} & \multicolumn{2}{c}{Dice Index $\uparrow$} &
    \multicolumn{2}{c}{Hausdorff $\downarrow$}\\
    \cmidrule{2-7}
    {}  & Part A & Part B & Part A & Part B & Part A & Part B\\
    \midrule
    DCAN~\cite{chen2016dcan}   
    & 0.912 & 0.716 & 0.897 & 0.781 & 45.42 & 160.35\\
    MCN~\cite{xu2017gland}  
    & 0.893 & 0.843 & 0.908 & 0.833 & 44.13 & 116.82\\
    SPL~\cite{yan2018deep}   & 0.924  & 0.844  & 0.902  & 0.840  & 49.88 & 106.08\\
    SA~\cite{yang2017suggestive} & 0.921 & 0.855 & 0.904 & 0.858 & 44.74 & 96.98\\
    FullNet~\cite{qu2019improving} & 0.924  & 0.853  & 0.914  & 0.856 & 37.28 & 88.75\\
    QSA~\cite{xu2018quantization} & 0.930 & 0.862 & 0.914 & {\bf 0.859} & 41.78 & 97.39\\
    \midrule
    SS & 0.872 & 0.765 & 0.853 & 0.797 & 54.86 & 116.33\\
    DT & 0.918 & 0.846 & 0.896 & 0.848 & 41.84 & 90.86\\
    \textbf{SDT} (Ours) & {\bf 0.931} & {\bf 0.866} & {\bf 0.919} 
    & 0.851 & {\bf 32.29} & {\bf 82.40}\\
    \bottomrule
    \end{tabular}}
    \end{center}
    \caption{Comparison with state-of-the-art methods on the gland segmentation challenge dataset. Our \sdt achieves better or on par F1 score and Dice Index, and significantly better Hausdorff distance for evaluating {\em shape similarity}. DT and SS represent distance transform and skeleton with scales, respectively.}\label{tab:gland}
\end{table}

==> tex-tab/tab_gland_ablation.tex <==
\begin{table}[t]
    \begin{center}
    \resizebox{0.7\columnwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{Setting} &  \multicolumn{2}{c}{F1 Score $\uparrow$} & \multicolumn{2}{c}{Dice Index $\uparrow$} &
    \multicolumn{2}{c}{Hausdorff $\downarrow$}\\
    \cmidrule{2-7}
    %\midrule
    {}  & Part A & Part B & Part A & Part B & Part A & Part B\\
    \midrule
    {\em Loss} \\
    L1 & 0.916 & 0.842 & 0.903 & 0.850 & 39.76 & 94.83\\
    L2 & 0.896 & 0.833 & 0.885 & 0.837 & 49.11 & 110.24\\
    CE & 0.931 & 0.866 & 0.919 & 0.851 & 32.29 & 82.40\\
    \midrule
    {\em Curvature} \\
    $\alpha=0.6$ & 0.912 & 0.845 & 0.914 & 0.855 & 36.25 & 91.24 \\
    $\alpha=0.8$ & 0.931 & 0.866 & 0.919 & 0.851 & 32.29 & 82.40 \\
    $\alpha=1.0$ & 0.926 & 0.858 & 0.907 & 0.849 & 35.73 & 86.73 \\
    \midrule
    {\em Skeleton} \\
    Partial & 0.899 & 0.831 & 0.896 & 0.837 & 47.50 & 105.19\\
    Local & 0.931 & 0.866 & 0.919 & 0.851 & 32.29 & 82.40 \\
    \bottomrule
    \end{tabular}}
    \end{center}
    \caption{Ablations studies on the gland dataset. The results suggest that the model trained with cross-entropy loss with $\alpha=0.8$ and local skeleton generation achieves the best performance.}\label{tab:gland_ablation}
\end{table}
